Lattice calculation of the short and intermediate time-distance hadronic vacuum polarization contributions to the muon magnetic moment using twisted-mass fermions

We present a lattice determination of the leading-order hadronic vacuum polarization (HVP) contribution to the muon anomalous magnetic moment, $a_{\mu}^{\rm HVP}$, in the so-called short and intermediate time-distance windows, $a_{\mu}^{\rm SD}$ and $a_{\mu}^{\rm W}$, defined by the RBC/UKQCD Collaboration [1]. We employ gauge ensembles produced by the Extended Twisted Mass Collaboration (ETMC) with $N_f = 2 + 1 + 1$ flavors of Wilson-clover twisted-mass quarks with masses of all the dynamical quark flavors tuned close to their physical values. The simulations are carried out at three values of the lattice spacing equal to $\simeq 0.057, 0.068$ and $0.080$ fm with spatial lattice sizes up to $L \simeq 7.6$~fm. For the short distance window we obtain $a_\mu^{\rm SD}({\rm ETMC}) = 69.27\,(34) \cdot 10^{-10}$, which is consistent with the recent dispersive value of $a_\mu^{\rm SD}(e^+ e^-) = 68.4\,(5) \cdot 10^{-10}$ [2]. In the case of the intermediate window we get the value $a_\mu^{\rm W}({\rm ETMC}) = 236.3\,(1.3) \cdot 10^{-10}$, which is consistent with the result $a_\mu^{\rm W}({\rm BMW}) = 236.7\,(1.4) \cdot 10^{-10}$ [3] by the BMW collaboration as well as with the recent determination by the CLS/Mainz group of $a_\mu^{\rm W}({\rm CLS}) = 237.30\,(1.46) \cdot 10^{-10}$ [4]. However, it is larger than the dispersive result of $a_\mu^{\rm W}(e^+ e^-) = 229.4\,(1.4) \cdot 10^{-10}$ [2] by approximately $3.6$ standard deviations. The tension increases to approximately $4.5$ standard deviations if we average our ETMC result with those by BMW and CLS/Mainz. Our accurate lattice results in the short and intermediate windows point to a possible deviation of the $e^+ e^-$ cross section data with respect to Standard Model predictions in the low and intermediate energy regions, but not in the high energy region.

==> charm.tex <==
\section{The charm-quark connected contribution to $a_\mu^{\rm SD}$ and $a_\mu^{\rm W}$}
\label{sec:charm}

Here we present the calculation of the charm-quark connected vector correlator (see Eq.\,(\ref{eq:Vregdetail}))
\be 
   V_{c}(t) \; \equiv \;  -\frac{1}{3} a^3\sum_{\bf x} \sum_{i=1,3} \frac{4}{9} \left\langle J_{i, reg}^{cc'}(x) [J_{i, reg}^{cc'}]^\dagger(0) \right\rangle^{\!(C)} \; ,  \quad reg \in \{ {\rm tm,OS} \, \} 
\ee
where the renormalized local vector currents $J_{\mu, tm}^{c c^\prime}$ and $J_{\mu, OS}^{c c^\prime}$ are defined in Eq.\,(\ref{eq:MAVcurr}). The suffix $c c'$ on the currents reminds that the quark and antiquark fields in each current correspond to different valence replica, giving rise to connected (label ($C$)) Wick contractions only.

%In this Section, we present the calculation of the charm-quark connected vector correlator $V_c(t)$ in the ``tm" and ``OS" regularizations, performed in an analogous manner as for the strange-quark case. %i.e.~by considering in Eq.\,(\ref{eq:Vrecomb}) the quark connected part of the insertions of the (renormalized) local vector currents $J_{\mu, tm}^{c c^\prime}$ and $J_{\mu, OS}^{c c^\prime}$ defined in Eq.\,(\ref{eq:MAVcurr}).
The charm-quark connected vector correlator $V_c(t)$ is computed using six ETMC ensembles. Beyond the three physical mass pion  ensembles, cB211.072.64, cC211.060.80 and cD211.054.96 listed in Table\,\ref{tab:simulated_mc}, we include in this analysis  three ensembles at a coarser lattice spacing, namely cA211.53.24, cA211.40.24 and cA211.30.32\,\cite{ExtendedTwistedMass:2021gbo, ExtendedTwistedMass:2021qui}, aiming at a better control of discretization effects in the charm sector\footnote{The  pion mass and the value of $M_\pi L$ for the cA211.53.24, cA211.40.24 and cA211.30.32 ensembles are equal to $M_\pi \simeq 365, 302, 261$ MeV and $M_\pi L \simeq 4.0, 3.5, 4.0$,  respectively. FSEs are expected to be negligible for the vector correlator $V_c(t)$ and thus, we do not include the cB211.072.96 ensemble in the charm analysis. We also expect the slight mistuning of the sea light-quark mass to have  a negligible effect. These expectations are fully confirmed by the results shown later in Figs.\,\ref{fig:SD_cont_lim_charm} and\,\ref{fig:W_cont_lim_charm}.}. The improved value of the lattice spacing $a$ for the A ensembles is given in Table\,\ref{tab:spacing}. 

Depending on the ensemble considered, up to $24$ spatial stochastic sources are used for the inversions of the Dirac operator. For each ensemble, we perform simulations at three values of the valence bare charm-quark mass, $a\mu_c$, in order to interpolate the results for $a_\mu^{\rm SD}(c)$ and $a_\mu^{\rm W}(c)$ to the physical charm-quark mass $m_c^{phys}$ {\bf as determined in Appendix\,\ref{sec:charm_mass}}.

In the top panels of Fig.~\ref{fig:VV_charm} we show the connected charm-quark vector correlators $V_c^{tm}(t)$ and $V_c^{OS}(t)$ obtained for two of the ETMC ensembles using, respectively, the renormalized local vector current $J_{\mu, tm}^{c c^\prime}$ and $J_{\mu, OS}^{c c^\prime}$. In the bottom panels we provide the same correlators after the subtraction of the perturbative lattice artifacts evaluated numerically at a finite bare quark mass equal to $\mu_c^L$ and lattice spacing $a$ in the free-theory, i.e.\,at order ${\cal{O}}(\alpha_s^0)$.
\begin{figure}[htb!]
\begin{center}
\includegraphics[scale=0.85]{VV_charm}
\caption{\it \small Top panels: the charm-quark connected vector correlator $t^3 V_c(t)$ corresponding to the ETMC ensembles cB211.072.64 and cD211.054.96 for the two regularizations, ``tm" and``OS", of the local vector current employed in this work versus the time distance $t$. For both ensembles the bare charm-quark mass is equal to $\mu_c = \mu_c^L$ (see Table\,\ref{tab:simulated_mc}). Bottom panels: the same as in the top panels, but after the subtraction of the perturbative lattice artifacts evaluated numerically at a finite bare quark mass equal to $\mu_c^L$ and lattice spacing $a$ in the free-theory.}
\label{fig:VV_charm}
\end{center}
\end{figure}
It can clearly be seen that the impact of the perturbative subtraction at order ${\cal{O}}(\alpha_s^0)$ is crucial for achieving a  reduction of the discretization effects in the two regularizations.

%In the following subsections we will interpolate/extrapolate our results for $a_\mu^{\rm SD}(c)$ and $a_\mu^{\rm W}(c)$ to the physical charm-quark mass point, determined from either the $\eta_c$- or the $J/\Psi$-meson mass as described in Appendix\,\ref{sec:charm_mass}. Then, we perform a separate continuum limit extrapolation for both determinations. Any discrepancy between the continuum extrapolated values obtained using the two hadronic inputs will be added as a systematic error in the final error budget. 




\subsection{Short-distance window: $a_\mu^{\rm SD}(c)$}
\label{sec:amuSD_c}

We  interpolate/extrapolate our data for $a_\mu^{\rm SD}(c)$ to the physical charm-quark mass $m_c^{phys}$ using a  linear Ansatz
\be
    a_\mu^{\rm SD}(c, m_c) = a_\mu^{\rm SD}(c, m_c^{phys}) \cdot \left[ 1 + A_c \left( m_c - m_c^{phys} \right) \right] ~    
\ee
with $a_\mu^{\rm SD}(c, m_c^{phys})$ and $A_c$ being free fitting parameters. 
In what follows we consider two different types of analysis, in which $a_\mu^{\rm SD}(c, m_c^{phys})$ is determined using the values of $m_c^{phys}$ from either the $\eta_c$ or the $J/\Psi$ meson masses.
The values of $a_\mu^{\rm SD}(c)$ obtained after the subtraction of the perturbative lattice artifacts at order $\mathcal{O}(\alpha_s^0)$ and after the interpolation/extrapolation to $m_c^{phys}$ are shown in Fig.~\ref{fig:SD_cont_lim_charm} for all the ETMC ensembles of Table~\ref{tab:simulated_mc} in the case of both the ``tm" and ``OS" regularizations, and for the two type of analyses in which we set the physical charm-quark mass using either the mass of the pseudoscalar $\eta_c$ meson or that of the vector $J/\Psi$ meson. The statistical errors of our lattice data for $a_\mu^{\rm SD}(c)$ are typically of order $\mathcal{O}(0.1 \%)$ for both choices of the reference hadron mass. No significant FSEs, as well as, no effects from the mistuning of the sea light-quark mass are visible within the errors for both regularizations. Discretization effects appear to be at the level of ${\cal{O}}(5 \%)$ with opposite signs between the ``tm" and ``OS" regularizations. The size of discretization effects is limited thanks to the subtraction of the perturbative cutoff effects at order ${\cal{O}}(\alpha_s^0)$ evaluated at the charm-quark mass.

In Fig.~\ref{fig:SD_cont_lim_strange} the solid lines correspond to the results of a  combined fit having the same structure as that of Eq.\,(\ref{eq:naive_fits}) for the light-quark case. The quality of the fits, including the quartic $a^4$ term for both regularizations, is quite good obtaining $\chi^2/d.o.f. \simeq 0.1~(0.4)$ when we use $M_{\eta_c}$ ($M_{J/\Psi}$). 
\begin{figure}[htb!]
\begin{center}
\includegraphics[scale=0.65]{SD_cont_lim_charm}
\caption{\it \small The charm-quark connected contribution to the short-distance window $a_\mu^{\rm SD}(c)$, versus the squared lattice spacing $a^2$ in physical units using both the ``tm" (squares) and ``OS" (triangles) local currents\, of Eq.~(\ref{eq:MAVcurr}) after subtraction of the perturbative lattice artifacts at order ${\cal{O}}(\alpha_s^0)$. The blue (red) points correspond to the lattice data obtained using the mass of the $\eta_c$ ($J/\Psi$) meson to obtain the physical charm-quark mass. The solid lines correspond to the results of the combined fitting procedure given in Eq.\,(\ref{eq:naive_fits}) including the quartic $a^4$ term for both regularizations. The extrapolated values are shown at $a^2 = 0$ together with our final result\,(\ref{eq:amuSD_charm_final}).}
\label{fig:SD_cont_lim_charm}
\end{center}
\end{figure}

We carry out several combined fits of our data adopting the general Ansatz described by Eq.~(\ref{eq:amuSD_fit}) in the light-quark case. As in the case of the strange-quark contribution, we set all the terms describing FSEs and the mistuning of the sea light-quark mass to zero in the case of $a_\mu^{\rm SD}(c)$.
In Fig.~\ref{fig:amuSD_strange}, we show some selected results obtained using different combined fits aiming at illustrating the spread between the various determinations. We show also the final error band determined by applying Eq.\,(\ref{eq:averaging}) to all the fits having $\chi^2/d.o.f.<1$, including also the spread due to the two type of analyses based on the $\eta_c$ and $J/\Psi$ meson masses. We carry out about 60 combined fits.
Our final result for $a_\mu^{\rm SD}(c)$ is
\be
    \label{eq:amuSD_charm_final}    
    a_\mu^{\rm SD}(c) = 11.64 ~ (10)_{stat} ~ (13)_{syst} \cdot 10^{-10} = 11.64 ~ (16) \cdot 10^{-10} ~ . ~    
\ee
\begin{figure}[htb!]
\begin{center}
\includegraphics[scale=0.50]{systematic_amu_SD_c}
\caption{\it \small Results of selected fits for $a_{\mu}^{\rm SD}(c)$ based on Eq.\,(\ref{eq:amuSD_fit}) and applied to our lattice data for the ETMC ensembles of Table\,\ref{tab:simulated_mc}, for the ``tm" and ``OS" regularizations and for the two type of the analyses corresponding to the use of either the $\eta_c$ or the $J/\Psi$ meson masses to set the physical charm-quark mass. The red band corresponds to our final result\,(\ref{eq:amuSD_charm_final}).}
\label{fig:amuSD_charm}
\end{center}
\end{figure}




\subsection{Intermediate window: $a_{\mu}^{\rm W}(c)$}
\label{sec:amuW_c}

As in the previous subsection, we have interpolated/extrapolated our lattice data for the charm-quark contribution to the intermediate window, $a_\mu^{\rm W}(c)$, to the physical charm-quark mass $m_c^{phys}$ using a linear Ansatz of the same type of Eq.\,(\ref{eq:aMP_fit_charm}).
As in the case of $a_\mu^{\rm SD}(c)$, we consider two different branches of the analysis, in which $a_\mu^{W}(c, m_c^{phys})$ is determined using the values of $m_c^{phys}$ from $M_{\eta_c}$ and from $M_{J/\Psi}$. 

Our lattice data for $a_\mu^{\rm W}(c)$, extrapolated to the physical charm-quark mass, are shown in Fig.~\ref{fig:W_cont_lim_charm} for the ETMC ensembles of Table~\ref{tab:simulated_mc}, for both ``tm" and ``OS" regularizations and for both choices of the reference hadron mass used to determine $m_c^{phys}$. 
In analogy with the case of the light-quark contribution to the intermediate window, we do not perform the subtraction of  cut-off effects at order ${\cal{O}}(\alpha_s^0)$. The results exhibit a very good precision of order $\mathcal{O}(0.5 \%)$ when we use $M_{\eta_c}$ and of order $\mathcal{O}(0.2 \%)$ when we use $M_{J/\Psi}$.  

In Fig.~\ref{fig:W_cont_lim_charm}, the solid lines correspond to the results of the combined fitting procedure having the same structure as that of Eq.\,(\ref{eq:naive_fits}) for the light-quark case. The quality of the fits is good obtaining $\chi^2/d.o.f. \simeq 0.1~(1.0)$ when we use $M_{\eta_c}$ ($M_{J/\Psi}$). As in the case of $a_\mu^{\rm SD}(c)$, we do not observe any FSEs and any effect of the mistuning of the sea light-quark mass is within the errors for both regularizations.
\begin{figure}[htb!]
\begin{center}
\includegraphics[scale=0.65]{W_cont_lim_charm}
\caption{\it \small The charm-quark connected contribution to the short time-distance window $a_\mu^{\rm W}(c)$, versus the squared lattice spacing $a^2$ in physical units using both the ``tm" (squares) and ``OS" (triangles) local currents\, defined in Eq.~(\ref{eq:MAVcurr}). The blue (red) points correspond to the lattice data obtained using the mass of the $\eta_c$ ($J/\Psi$) meson to determine the physical charm-quark mass. The solid lines correspond to the results of the combined fitting procedure given in Eq.\,(\ref{eq:naive_fits}) with the quartic $a^4$ terms included for both regularizations. The extrapolated values are shown at $a^2 = 0$ together with our final result\,(\ref{eq:amuW_charm_final}).}
\label{fig:W_cont_lim_charm}
\end{center}
\end{figure}

In Fig.~\ref{fig:amuW_strange}, we present selected results obtained using different combined fits in order to illustrate the spread among the various determinations. We show also the final error band determined by applying Eq.~(\ref{eq:averaging}) to the fits leading to $\chi^2/d.o.f.<1.8$. The total number of the combined fits performed for $a_\mu^{\rm W}(c)$ is about 60. 
\begin{figure}[htb!]
\begin{center}
\includegraphics[scale=0.50]{systematic_amu_W_c}
\caption{\it \small Results of selected fits for $a_\mu^{\rm W}(c)$ based on Eq.\,(\ref{eq:amuW_fit}) and applied to our lattice data for all the ETMC ensembles of Table\,\ref{tab:simulated_mc}, for the ``tm" and ``OS" regularizations and for the two type of  analyses corresponding to the use of either the $\eta_c$ or the $J/\Psi$ meson masses to set the physical charm-quark mass. The red band corresponds to our final result\,(\ref{eq:amuW_charm_final}).}
\label{fig:amuW_charm}
\end{center}
\end{figure}

The extracted value for $a_\mu^{\rm W}(c)$ is
\be
    \label{eq:amuW_charm_final}    
    a_\mu^{\rm W}(c) = 2.95 ~ (4)_{stat} ~ (12)_{syst} \cdot 10^{-10} = 2.95 ~ (13) \cdot 10^{-10} ~ . ~   
\ee

